Caught in the Game: On the History and Evolution of Web Browser Gaming

Web browsers have come a long way since their inception, evolving from a simple means of displaying text documents over the network to complex software stacks with advanced graphics and network capabilities. As personal computers grew in popularity, developers jumped at the opportunity to deploy cross-platform games with centralized management and a low barrier to entry. Simply going to the right address is now enough to start a game. From text-based to GPU-powered 3D games, browser gaming has evolved to become a strong alternative to traditional console and mobile-based gaming, targeting both casual and advanced gamers. Browser technology has also evolved to accommodate more demanding applications, sometimes even supplanting functions typically left to the operating system. Today, websites display rich, computationally intensive, hardware-accelerated graphics, allowing developers to build ever-more impressive applications and games.In this paper, we present the evolution of browser gaming and the technologies that enabled it, from the release of the first text-based games in the early 1990s to current open-world and game-engine-powered browser games. We discuss the societal impact of browser gaming and how it has allowed a new target audience to accessdigital gaming. Finally, we review the potential future evolution ofthe browser gaming industry.

==> latexmkrc <==
$pdf_mode = 1;

add_cus_dep('gnuplot', 'eps', 0, 'gnuplot_to_eps');
sub gnuplot_to_eps {
    system("gnuplot \"$_[0].gnuplot\"");
}

